Recall Traces: Backtracking Models for Efficient Reinforcement Learning

In many environments only a tiny subset of all states yield high reward. In these cases, few of the interactions with the environment provide a relevant learning signal. Hence, we may want to preferentially train on those high-reward states and the probable trajectories leading to them. To this end, we advocate for the use of a backtracking model that predicts the preceding states that terminate at a given high-reward state. We can train a model which, starting from a high value state (or one that is estimated to have high value), predicts and sample for which the (state, action)-tuples may have led to that high value state. These traces of (state, action) pairs, which we refer to as Recall Traces, sampled from this backtracking model starting from a high value state, are informative as they terminate in good states, and hence we can use these traces to improve a policy. We provide a variational interpretation for this idea and a practical algorithm in which the backtracking model samples from an approximate posterior distribution over trajectories which lead to large rewards. Our method improves the sample efficiency of both on- and off-policy RL algorithms across several environments and tasks.

==> rl_adv.tex <==
\section{Current Implementation}

\begin{itemize}
    \item First step is to somehow get high value states or "sub-goals"
    \item Learn a backwards model using the trajectories which leads to high value states.
    \item Sample trajectory from the backwards model
    \item Increase the likelihood of the states visited by the backwards model under the forward policy.
\end{itemize}


\section{A new learning rule for Reinforcement Learning }

Lets begin by formalizing the learning algorithm. Given an input $s \in S$ from the
environment, the policy has to select an action $a \in A$ and then receives
a scalar reward signal r, with a  distribution that depend on state s and action a. The goal of the learning algorithm  is to choose an output which maximizes the expected
reward. Due to the lack of an explicit error signal, the learner must choose its
output stochastically, exploring for better rewards. 


Typically the learner starts with
a parameterized form for the conditional output density $P_\theta(a|s)$, and the learning
problem becomes one of finding the parameters $\theta$ which maximize the expected
reward: 

$$ J_r(\theta)=\int_{S,A} p(s) p_\theta(a|s) \overline{{r}}(s,a)  da ds$$

The policy task is to choose from a set of conditional output distributions based
on the reward it receives from the environment. These rewards can be thought of as
inverse energies; input/output pairs that receive high rewards are low energy and
are preferred by the environment. Energies can always be converted into probabilities
through the Boltzmann distribution, and so we can define the environment's
conditional distribution on A given s, 

$$ p^{*}(a|s) = \frac{exp(-T^{-1}E(s,a))}{Z_{T}(x)} = \frac{exp(-T^{-1}\overline{r}(s,a))}{Z_{T}(x)} $$

where T is a temperature parameter and $Z_T(X)$ is a normalization constant which
depends on T . This distribution can be thought of as representing the environment's
ideal input-output mapping, high reward input-output pairs being more typical or
likely than low reward pairs. 

The temperature parameter determines the strength of this preference: 
\begin{itemize}
    \item When T is infinity all outputs are equally likely.
    \item When T is zero only the highest reward output is chosen.
\end{itemize}
This new distribution is a purely theoretical
construct, but it can be used as a target distribution for the policy. If the $\theta$ are
adjusted so that $p_\theta(a|s)$ is nearly equal to $p^{*}(a|s)$, then the network's output will
typically result in high rewards.

The agreement between the network and environment conditional output densities
can be measured with the Kullback-Liebler (KL) divergence: 

$$KL(p|p^{*}) = - \int_{S,A} p(s) p_\theta(a|s) [log (p^{*}(a|s)) -log(p_\theta(a|s))] da ds $$

$$ = - 1/T \int_{S,A} p(s) p_\theta(a|s) [r(s,a) - T\hat{r}_{\theta}(s,a)] da ds $$

$$ = - \int_{S,A} p(s) p_\theta(a|s) [r(s,a) - T\hat{r}_{\theta}(s,a)] da ds $$

$$ = - J_r(\theta) - TS(p_\theta)$$

where $r_\theta(s, a)$ is defined as the logarithm of the conditional output probability and can be thought of as the network's estimate of the mean reward. This cost function
is always greater than or equal to zero, with equality only when the two probability
distributions are identical. 

The new cost function is analogous to a free energy, balancing the energy, in the
form of the negative of the average reward, and the entropy $S(p_\theta)$ of the output distribution. 
\begin{itemize}
    \item A higher T corresponds to a smoother target distribution and tilts the
balance of the cost function in favor of the entropy term, making diffuse output distributions
more favorable.
    \item  A small T results in a sharp target distribution
placing most of the weight on the reward dependent term of cost function, which is
always optimized by the singular solution of a spike at the highest reward output.
\end{itemize}

Although minimizing the new cost function will result in sampling most often at
high reward outputs, it will not optimize the overall expected reward if $T > O$.
There are two reasons for this. 
\begin{itemize}
\item  First, the output a which maximizes $\bar{r}(s, a)$ may
not maximize $\overline{r}(s, a)$. The network will/might choose outputs which are suboptimal
with respect to its own predicted reward. BUT The key point here is that early in learning
this non-optimality is exactly what is desired. The new cost function forces the
learner to maintain output density everywhere the reward is not much smaller than its maximum. When T is high, the rewards are effectively
flattened and even fairly small rewards look big. This means that a high temperature
ensures that the learner will explore the output space.
\item Once the network is nearly  optimal, it would be advantageous to "sharpen up"
the conditional output distribution, sampling more often at outputs with higher
predicted rewards. This translates to decreasing the entropy of the output distribution
or lowering T.

\end{itemize}

The idea of the
the proposed algorithm is to begin training with a large T, say unity, and
gradually decrease it as the performance improves, effectively shifting the bias of
the learner from exploration to exploitation. 

The advantage of the
proposed learning rule is that it allows for an early training phase which encourages exploration without forcing the output distribution to converge on suboptimal outputs.

\section{Connections to what I'm doing now}

If we assume $p_\theta$ refers to the backwards model, then I'm essentially optimizing the proposed cost function.
The way I am implementing is that I'm learning the backwards \textbf{only} using the trajectories which leads to high values states. And once I learned this backwards model, I start the backwards model from high value state (i.e very low temperature i.e I sharpen the conditional output distribution by starting the backwards model from \textbf{high value state}, and then I increase the likelihood of the states visited by the backwards model under the forward policy. Hence, if my analysis is correct, the way I've implemented this, is only doing \textbf{exploitation} and no exploration at all. 

% \section{How to change the training algorithm to accommodate this "temperature" formulation}

% Anirudh does not know how to do that right now.

% \section{Proposed Algorithm in Variational Framework}

% Anirudh has to think more about it. And write it down. 

% \section{Neuroscience Connection}

